Randomized HyperSteiner: A Stochastic Delaunay Triangulation Heuristic for the Hyperbolic Steiner Minimal Tree

We study the problem of constructing Steiner Minimal Trees (SMTs) in hyperbolic space. Exact SMT computation is NP-hard, and existing hyperbolic heuristics such as HyperSteiner are deterministic and often get trapped in locally suboptimal configurations. We introduce Randomized HyperSteiner (RHS), a stochastic Delaunay triangulation heuristic that incorporates randomness into the expansion process and refines candidate trees via Riemannian gradient descent optimization. Experiments on synthetic data sets and a real-world single-cell transcriptomic data show that RHS outperforms Minimum Spanning Tree (MST), Neighbour Joining, and vanilla HyperSteiner (HS). In near-boundary configurations, RHS can achieve a 32% reduction in total length over HS, demonstrating its effectiveness and robustness in diverse data regimes.

==> sections/checklist.tex <==
\newpage
\section*{Checklist}

% % %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references. For each question, choose your answer from the three possible options: Yes, No, Not Applicable.  You are encouraged to include a justification to your answer, either by referencing the appropriate section of your paper or providing a brief inline description (1-2 sentences). 
% Please do not modify the questions.  Note that the Checklist section does not count towards the page limit. Not including the checklist in the first submission won't result in desk rejection, although in such case we will ask you to upload it during the author response period and include it in camera ready (if accepted).

% \textbf{In your paper, please delete this instructions block and only keep the Checklist section heading above along with the questions/answers below.}

% [Yes/No/Not Applicable]
% % %%% END INSTRUCTIONS %%%


\begin{enumerate}

  \item For all models and algorithms presented, check if you include:
  \begin{enumerate}
    \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. 
    
    \textit{Answer:} \textbf{[Yes]}. 
    
    \textit{Justification:} Section~\ref{sec:bg} provides comprehensive background on the Klein-Beltrami model, Steiner Minimal Trees, and Delaunay triangulation. Section~\ref{sec:meth} details the method with Algorithm~\ref{alg:rad_hyper}, and Appendix~\ref{app:heuristic} provides additional implementation details (Algorithms~\ref{alg:red}-\ref{alg:edge-in}).
    
    \item An analysis of the properties and complexity (time, space, sample size) of any algorithm.

    \textit{Answer:} \textbf{[Yes]}. 
    
    \textit{Justification:}  Appendices~\ref{app:heuristic} and \ref{app:og_hyp} provide theoretical complexity analysis of main algorithm components, while Appendix~\ref{app:exp} presents detailed empirical runtime measurements across varying problem sizes and includes an extended scalability discussion.

    
    \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. 

    \textit{Answer:} \textbf{[Yes]}. 
    
    \textit{Justification:}  As stated in Section~\ref{sec:exp}, the source code and experiment scripts are available in the Supplementary Material.
    
  \end{enumerate}

  \item For any theoretical claim, check if you include:
  \begin{enumerate}
    \item Statements of the full set of assumptions of all theoretical results. 

     \textit{Answer:} \textbf{[Yes]}. 
    
    \textit{Justification:}  Theorem~\ref{thm:uniqueness} clearly states assumptions (fixed terminal points in Klein disk, fixed tree topology). Proposition~\ref{prop:isoptic} and other theoretical results explicitly state their prerequisites.


    
    \item Complete proofs of all theoretical results. 

     \textit{Answer:} \textbf{[Yes]}. 
    
    \textit{Justification:}  Appendix~\ref{app:uniq} provides complete proofs including Lemma~\ref{lem:segment_isoptic}, Theorem~\ref{thm:uniqueness}, and Lemma~\ref{lem:model_independence}. Other results contain citations to references with their corresponding proofs.

    
    \item Clear explanations of any assumptions.

    \textit{Answer:} \textbf{[Yes]}. 
    
    \textit{Justification:}  Appendix~\ref{app:uniq} provides complete proofs including Lemma~\ref{lem:segment_isoptic}, Theorem~\ref{thm:uniqueness}, and Lemma~\ref{lem:model_independence}. Other results contain citations to references with their corresponding proofs.

  \end{enumerate}

  \item For all figures and tables that present empirical results, check if you include:
  \begin{enumerate}
    \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). 
    
    
    \textit{Answer:} \textbf{[Yes]}. 
    
    \textit{Justification:}  As stated in Section~\ref{sec:exp}, the source code and experiment scripts are available in the Supplementary Material.
    
    \item All the training details (e.g., data splits, hyperparameters, how they were chosen). 

       \textit{Answer:} \textbf{[Yes]}. 
    
    \textit{Justification:} Details regarding the experimental section configuration can be found in Section~\ref{sec:exp}, as well as in Appendix~\ref{app:exp_det}.

    
    \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). 

         \textit{Answer:} \textbf{[Yes]}. 
    
    \textit{Justification:} For each experiment, results are averaged over 10 independent samplings, reporting mean reduction over MST (RED,~\%) with standard deviation.



    
    \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider).

  \textit{Answer:} \textbf{[Yes]}. 
    
    \textit{Justification:}  As stated in Section~\ref{sec:exp}, all the experiments were conducted on Google Cloud (n2d CPUs, 1 core, 128GB RAM).
    
  \end{enumerate}

  \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
  \begin{enumerate}
    \item Citations of the creator If your work uses existing assets. 

 \textit{Answer:} \textbf{[Yes]}. 
    
    \textit{Justification:}  The paper properly cites: \cite{garcia2025hypersteiner} for HyperSteiner, \cite{Plass2018_planaria_SingleCellData} for the Planaria dataset and \cite{Klimovskaia2020SingleCellPoincareMap} for its hyperbolic embedding, \cite{Saitou1987neighborjoining} for Neighbour Joining, and all other methods/datasets used.
    
    \item The license information of the assets, if applicable. 


 \textit{Answer:} \textbf{[Not Applicable]}. 
    
    \textit{Justification:}   All the used assets are available under Creative Commons Attribution (CC BY) licenses, which permit reuse with appropriate citation as provided in the references.
    
    \item New assets either in the supplemental material or as a URL, if applicable.  
    
    \textit{Answer:} \textbf{[Yes]}. 
    
    \textit{Justification:}  Code and scripts mentioned in supplementary material.

    
    \item Information about consent from data providers/curators.  
    
         \textit{Answer:} \textbf{[Not Applicable]}. 

    \textit{Justification:}  All the used assets are available under Creative Commons Attribution (CC BY) licenses, which permit reuse with appropriate citation as provided in the references.
    

    
    \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. 


     \textit{Answer:} \textbf{[Not Applicable]}. 
    
    \textit{Justification:}  
    The paper uses synthetic data and single-cell RNA-sequencing data with no PII or sensitive content.
    

  \end{enumerate}


  \item If you used crowdsourcing or conducted research with human subjects, check if you include:
  \begin{enumerate}
    \item The full text of instructions given to participants and screenshots.

  \textit{Answer:} \textbf{[Not Applicable]}. 
    
    \textit{Justification:}  This is a purely computational/algorithmic study with no human subjects or crowdsourcing.
    
    \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable.

          \textit{Answer:} \textbf{[Not Applicable]}. 
    
    \textit{Justification:}  This is a purely computational/algorithmic study with no human subjects or crowdsourcing.

    
    \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. 


      \textit{Answer:} \textbf{[Not Applicable]}. 
    
    \textit{Justification:}  This is a purely computational/algorithmic study with no human subjects or crowdsourcing.
  \end{enumerate}

\end{enumerate}
